Modelling interactions between active and passive agents moving through heterogeneous environments

We study the dynamics of interacting agents from two distinct inter-mixed populations: One population includes active agents that follow a predetermined velocity field, while the second population contains exclusively passive agents, i.e. agents that have no preferred direction of motion. The orientation of their local velocity is affected by repulsive interactions with the neighboring agents and environment. We present two models that allow for a qualitative analysis of these mixed systems. We show that the residence times of this type of systems containing mixed populations is strongly affected by the interplay between these two populations. After showing our modeling and simulation results, we conclude with a couple of mathematical aspects concerning the well-posedness of our models.

==> Crowd dynamics book chapter/reference.tex <==

%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
%\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{Bensoussan1995} A. Bensoussan: Stochastic Navier-Stokes equations. Acta Applicandae Mathematicae \textbf{38}, pp. 59-85 (1995)
\bibitem{Boyer2013} F. Boyer, P. Fabrie: Mathematical tools for the Study of the Incompressible Navier-Stokes Equations and Related Models. Springer New York Heidelberg Dordrecht London (2013)
\bibitem{Billingsley1999} P. Billingsley: Convergence of Probability Measures. Wiley series in Probability and Statistics (1999)
\bibitem{Cialela} A. Cialela,  E. N. M. Cirillo, P. L. Cur\c seu, A. Muntean : Free to move or trapped in your group:
Mathematical modeling of information overload and coordination in
crowded populations, to appear in Mathematical Models and Methods in Applied Sciences  M3AS (2018)
\bibitem{Evans1997} L. C. Evans: Partial Differential Equations. American Mathematical Society (1997)
\bibitem{Flandoli95} F. Flandoli, D. Gatarek: Martingale and Stationary solutions for stochastic Navier-Stokes equations. Probability Theory and Related Fields \textbf{102}, pp. 367-391 (1995)
\bibitem{Jacod2004} J. Jacod, P. Protter: Probability Essentials. Springer (2004)
\bibitem{Prato14} G. Da Prato, J. Zabczyk: Stochastic equation in infinite dimensions. Encyclopedia of Mathematics and Its Applications (2014)
\bibitem{Adams03} R. A. Adams, J. J. F. Fourier: Sobolev Space. Elsevier (2013)
\bibitem{Pankavich15} S. Pankavich, N. Michalowski: A short proof of increased parabolic regularity. Electronic Journal of Differential Equations \textbf{2005}(2005), pp. 1-9 (2015)
\bibitem{Omar2017} 
O. Richardson, A. Jalba, A. Muntean: Effects of environment knowledge in evacuation scenarios involving fire and smoke - a multiscale modelling and simulation approach. (2017)
\url{https://arxiv.org/pdf/1709.07786.pdf}
\bibitem{Nguyen2013} M. H. Nguyen, T. V. Ho, J. D. Zucker: Integration of Smoke Effect and Blind Evacuation Strategy (SEBES) within fire evacuation simulation. Simulation Modelling Practice and Theory \textbf{36}, pp. 44-59  (2013)
\bibitem{Nguyen2015} M. H. Nguyen, T. V. Ho, J. C. Richaud: Modeling and Simulation of Fire Evacuation in Public Buildings. ACSIJ Advances in Computer Science: an International Journal, \textbf{6}, pp. 1-7 (2015) 
\bibitem{Anh2012} N. T. N. Anh, Z. J. Daniel, N. H. Du, A. Drogoul, V. D. An: A Hybrid Macro-Micro Pedestrians Evacuation Model to Speed Up Simulation in Road Networks. AAMAS 2011 Workshops, \textbf{7068}, pp. 371-383 (Springer-Verlag Berlin Heidelberg 2012)
\bibitem{Chu2014} M. L. Chu, P. Parigi, K. Law, J. C. Latombe: Modeling social behaviors in an evacuation simulator. Computer Animation and Virtual Worlds \textbf{25}, pp. 373-382  (2014)
\bibitem{Tsai2011} J. Tsai, N. Fridman, E. Bowring, M. Brown, S. Epstein, G. Kaminka, S. Marsella, A. Ogden, I. Rika, A. Sheel, M. Taylor, X. Wang, A. Zilka, M. Tambe :ESCAPES-Evacuation Simulation with Children,
Authorities, Parents, Emotions, and Social comparison. Proc. of The 10th International Conference on Autonomous Agents and Multiagent Systems (Taipei, Taiwan) \textbf{2}, pp. 457-464 (2011)
\bibitem{Horiuchi1986} S. Horiuchi, Y. Murozaki, A. Hukugo: A case study of fire and evacuation in a
multi-purpose office building, Osaka, Japan. Fire Safety Science, \textbf{1}, pp. 523-532 (1986)
\bibitem{Pavliotis2014} G. A. Pavliotis: Stochastic Processes and Applications: Diffusion Processes, the Fokker Planck and Langevin Equations. Springer Science + Business Media New York (2014)
\bibitem{Cristiani2014} E. Cristiani, B. Piccoli, A. Tosin: Multiscale Modeling of Pedestrian Dynamics. Springer International Publishing Switzerland (2014)
\bibitem{Evans2013} L. C. Evans: An Introduction to Stochastic Differential Equations. American Mathematical Society (2013)
\bibitem{Colombo2011} R. M. Colombo, M. Gagavello, M. L. Mercier: Non-local crowd dynamics. Comptes Rendus Mathematique, \textbf{349}, pp. 769-772 (2011)
\bibitem{Colombo2014} R. M. Colombo, F. Marcellini: A mixed ODE-PDE model for vehicular traffic. Mathematical Methods in the Applied Sciences, \textbf{38}, pp. 1292-1302 (2015)
\bibitem{Colombo2015_1} R. Borsche, R. M. Colombo, M. Garavello, A. Meurer: Differential Equations Modeling Crowd Interactions. Journal of Nonlinear Science, \textbf{25}, pp. 827-859 (2015)
\bibitem{Colombo2015_2} R. M. Colombo, T. Lorenz, N. I. Pogodaev: On the modeling of moving populations through set evolution equations. Discrete and Continuous Dynamical Systems - A, \textbf{35}(1), pp. 73-98 (2015)
\bibitem{Bellomo2013} N. Bellomo, A. Bellouquid, D. Knopoff: From the Microscale to Collective Crowd Dynamics. Multiscale Modeling and Simulation, \textbf{11}(3), pp. 943-963 (2013)
\bibitem{Bellomo2015} N. Bellomo, L. Gibelli: Toward a mathematical theory of behavioral-social dynamics for pedestrian crowds. Mathematical Models and Methods in Applied Sciences, \textbf{25}, pp. 2417-2437 (2015)
\bibitem{Bellomo2016_1} N. Bellomo, D. Clarke, L. Gibelli, P. Townsend, B. J. Vreugdenhil: Human behaviours in evacuation crowd dynamics: From modelling to “big data” toward crisis management. Physics of Life Reviews, \textbf{18}, pp. 1-21 (2016)
\bibitem{Bellomo2016_2} N. Bellomo, L.Gibelli: Behavioral crowds: Modeling and Monte Carlo simulations toward validation. Computers and Fluids, \textbf{141}, pp. 13-21 (2016)
\bibitem{Bellomo2016_3} N. Bellomo, S. Berrone, L. Gibelli, A. B. Pieri: Macroscopic First Order Models of Multicomponent Human Crowds with Behavioral Dynamics. In: Y. Bazilevs, K. Takizawa (eds). Advances in Computational Fluid-Structure Interaction and Flow Simulation. Modeling in Science, Engineering and Technology. Brikh\''{a}user, Cham (2016)
\bibitem{Bellomo2008} N. Bellomo: Modeling Crowds and Swarms:Congested and Panic Flows. In: Modeling Complex Living Systems. Modeling and Simulation in Science, Engineering and Technology. Birkh\''{a}user Boston (2008)
\bibitem{Bellomo2017} N. Bellomo, A. Bellouquid, L. Gibelli, N. Outada: Mathematical Models of Crowd Dynamics in Complex Venues. In: A Quest Towards a Mathematical Theory of Living Systems. Modeling and Simulation in Science, Engineering and Technology. Brikh\''{a}user, Cham (2017)
\bibitem{Cristiani2011} E. Cristiani, B. Piccoli, A. Tosin: Multiscale modeling of granular flows with application to crowd dynamics. Multiscale Modeling and Simulation, \textbf{9}(1), pp. 155-182 (2011)
\bibitem{Piccoli2009} B. Piccoli, A. Tosin: Pedestrian flows in bounded domains with obstacles. Continuum Mechanics and Thermodynamics, \textbf{21}, pp. 85-107 (2009)
\bibitem{Zuriguel2014} I. Zuriguel, D. R. Parisi, R. C. Hidalgo, C. Lozano, A. Janda, P. A. Gago, J. P. Peralta, L. M. Ferrer, L. A. Pugnaloni, E. Cl\'{e}ment, D. Maza, I. Pagonabarraga, A. Garcimart\'{i}n: Clogging transition of many-particle systems flowing through bottlenecks. Scientific Reports, \textbf{4}, 7324 (2014)
\bibitem{Garcimartin2015} A. Garcimart\'{i}n, J. M. Pastor, L. M. Ferrer, J. J. Ramos, C. Mart\'{i}n-G\'{o}mez, I. Zuriguel: Flow and clogging of a sheep herd passing through a bottleneck. Physical Review E, \textbf{91}, 022808 (2015)
\bibitem{OmarMSC} O.  Richardson: Large-scale multiscale particle models in inhomogeneous domains: modelling and implementation. Master thesis (2016) \url{https://arxiv.org/abs/1609.03732} 
\bibitem{Faure2015} S. Faure, B. Maury: Crowd motion from the granular stand point. Mathematical Models and Methods in Applied Sciences, \textbf{25} pp. 463-493 (2015)
\bibitem{Bortz} A.B.Bortz, M.H.Kalos, J.L.Lebowitz: New algorithm for Monte Carlo simulations of Ising spin systems. J. Comp. Phys. \textbf{17}, pp. 10-18 (1975)
\bibitem{Kratzer} P. Kratzer: Monte Carlo and Kinetic Monte Carlo. Methods -- A Tutorial, in Multiscale Simulation Methods in Molecular Sciences, edited by J. Grotendorst, N. Attig, S. Blügel, and D. Marx, NIC Series (Forschungszentrum Jülich), \textbf{42}, pp. 51-76 (2009)


% Journal article
%\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%%
%% Journal article by DOI
%\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%%
%\bigskip
%
%% Use the following (APS) syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Mathematics, Physics, Statistics, Computer Science"
%%
%% Online Document
%\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%%
%% Monograph
%\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%%
%% Journal article
%\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%%
%% Journal article by DOI
%\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%%
%% Contribution 
%\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%%
%\bigskip
%%
%% Use the following syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Psychology, Social Sciences"
%%
%%
%% Monograph
%\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%%
%% Online Document
%\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%%
%% Journal article
%\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
%\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
%\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
%\bigskip
%
% Journal article
%\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
%\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
%\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
%\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
%\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O�Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...�': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
%\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
%\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
%\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
%\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
%\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
%\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> reference.tex <==

%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
%\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{Bensoussan1995} A. Bensoussan: Stochastic Navier-Stokes equations. Acta Applicandae Mathematicae \textbf{38}, pp. 59-85 (1995)
\bibitem{Boyer2013} F. Boyer, P. Fabrie: Mathematical tools for the Study of the Incompressible Navier-Stokes Equations and Related Models. Springer New York Heidelberg Dordrecht London (2013)
\bibitem{Billingsley1999} P. Billingsley: Convergence of Probability Measures. Wiley series in Probability and Statistics (1999)
\bibitem{Cialela} A. Cialela,  E. N. M. Cirillo, P. L. Cur\c seu, A. Muntean : Free to move or trapped in your group:
Mathematical modeling of information overload and coordination in
crowded populations, to appear in Mathematical Models and Methods in Applied Sciences  M3AS (2018)
\bibitem{Evans1997} L. C. Evans: Partial Differential Equations. American Mathematical Society (1997)
\bibitem{Flandoli95} F. Flandoli, D. Gatarek: Martingale and Stationary solutions for stochastic Navier-Stokes equations. Probability Theory and Related Fields \textbf{102}, pp. 367-391 (1995)
\bibitem{Jacod2004} J. Jacod, P. Protter: Probability Essentials. Springer (2004)
\bibitem{Prato14} G. Da Prato, J. Zabczyk: Stochastic equation in infinite dimensions. Encyclopedia of Mathematics and Its Applications (2014)
\bibitem{Adams03} R. A. Adams, J. J. F. Fourier: Sobolev Space. Elsevier (2013)
\bibitem{Pankavich15} S. Pankavich, N. Michalowski: A short proof of increased parabolic regularity. Electronic Journal of Differential Equations \textbf{2005}(2005), pp. 1-9 (2015)
\bibitem{Omar2017} 
O. Richardson, A. Jalba, A. Muntean: Effects of environment knowledge in evacuation scenarios involving fire and smoke - a multiscale modelling and simulation approach. (2017)
\url{https://arxiv.org/pdf/1709.07786.pdf}
\bibitem{Nguyen2013} M. H. Nguyen, T. V. Ho, J. D. Zucker: Integration of Smoke Effect and Blind Evacuation Strategy (SEBES) within fire evacuation simulation. Simulation Modelling Practice and Theory \textbf{36}, pp. 44-59  (2013)
\bibitem{Nguyen2015} M. H. Nguyen, T. V. Ho, J. C. Richaud: Modeling and Simulation of Fire Evacuation in Public Buildings. ACSIJ Advances in Computer Science: an International Journal, \textbf{6}, pp. 1-7 (2015) 
\bibitem{Anh2012} N. T. N. Anh, Z. J. Daniel, N. H. Du, A. Drogoul, V. D. An: A Hybrid Macro-Micro Pedestrians Evacuation Model to Speed Up Simulation in Road Networks. AAMAS 2011 Workshops, \textbf{7068}, pp. 371-383 (Springer-Verlag Berlin Heidelberg 2012)
\bibitem{Chu2014} M. L. Chu, P. Parigi, K. Law, J. C. Latombe: Modeling social behaviors in an evacuation simulator. Computer Animation and Virtual Worlds \textbf{25}, pp. 373-382  (2014)
\bibitem{Tsai2011} J. Tsai, N. Fridman, E. Bowring, M. Brown, S. Epstein, G. Kaminka, S. Marsella, A. Ogden, I. Rika, A. Sheel, M. Taylor, X. Wang, A. Zilka, M. Tambe :ESCAPES-Evacuation Simulation with Children,
Authorities, Parents, Emotions, and Social comparison. Proc. of The 10th International Conference on Autonomous Agents and Multiagent Systems (Taipei, Taiwan) \textbf{2}, pp. 457-464 (2011)
\bibitem{Horiuchi1986} S. Horiuchi, Y. Murozaki, A. Hukugo: A case study of fire and evacuation in a
multi-purpose office building, Osaka, Japan. Fire Safety Science, \textbf{1}, pp. 523-532 (1986)
\bibitem{Pavliotis2014} G. A. Pavliotis: Stochastic Processes and Applications: Diffusion Processes, the Fokker Planck and Langevin Equations. Springer Science + Business Media New York (2014)
\bibitem{Cristiani2014} E. Cristiani, B. Piccoli, A. Tosin: Multiscale Modeling of Pedestrian Dynamics. Springer International Publishing Switzerland (2014)
\bibitem{Evans2013} L. C. Evans: An Introduction to Stochastic Differential Equations. American Mathematical Society (2013)
\bibitem{Colombo2011} R. M. Colombo, M. Gagavello, M. L. Mercier: Non-local crowd dynamics. Comptes Rendus Mathematique, \textbf{349}, pp. 769-772 (2011)
\bibitem{Colombo2014} R. M. Colombo, F. Marcellini: A mixed ODE-PDE model for vehicular traffic. Mathematical Methods in the Applied Sciences, \textbf{38}, pp. 1292-1302 (2015)
\bibitem{Colombo2015_1} R. Borsche, R. M. Colombo, M. Garavello, A. Meurer: Differential Equations Modeling Crowd Interactions. Journal of Nonlinear Science, \textbf{25}, pp. 827-859 (2015)
\bibitem{Colombo2015_2} R. M. Colombo, T. Lorenz, N. I. Pogodaev: On the modeling of moving populations through set evolution equations. Discrete and Continuous Dynamical Systems - A, \textbf{35}(1), pp. 73-98 (2015)
\bibitem{Bellomo2013} N. Bellomo, A. Bellouquid, D. Knopoff: From the Microscale to Collective Crowd Dynamics. Multiscale Modeling and Simulation, \textbf{11}(3), pp. 943-963 (2013)
\bibitem{Bellomo2015} N. Bellomo, L. Gibelli: Toward a mathematical theory of behavioral-social dynamics for pedestrian crowds. Mathematical Models and Methods in Applied Sciences, \textbf{25}, pp. 2417-2437 (2015)
\bibitem{Bellomo2016_1} N. Bellomo, D. Clarke, L. Gibelli, P. Townsend, B. J. Vreugdenhil: Human behaviours in evacuation crowd dynamics: From modelling to “big data” toward crisis management. Physics of Life Reviews, \textbf{18}, pp. 1-21 (2016)
\bibitem{Bellomo2016_2} N. Bellomo, L.Gibelli: Behavioral crowds: Modeling and Monte Carlo simulations toward validation. Computers and Fluids, \textbf{141}, pp. 13-21 (2016)
\bibitem{Bellomo2016_3} N. Bellomo, S. Berrone, L. Gibelli, A. B. Pieri: Macroscopic First Order Models of Multicomponent Human Crowds with Behavioral Dynamics. In: Y. Bazilevs, K. Takizawa (eds). Advances in Computational Fluid-Structure Interaction and Flow Simulation. Modeling in Science, Engineering and Technology. Brikh\''{a}user, Cham (2016)
\bibitem{Bellomo2008} N. Bellomo: Modeling Crowds and Swarms:Congested and Panic Flows. In: Modeling Complex Living Systems. Modeling and Simulation in Science, Engineering and Technology. Birkh\''{a}user Boston (2008)
\bibitem{Bellomo2017} N. Bellomo, A. Bellouquid, L. Gibelli, N. Outada: Mathematical Models of Crowd Dynamics in Complex Venues. In: A Quest Towards a Mathematical Theory of Living Systems. Modeling and Simulation in Science, Engineering and Technology. Brikh\''{a}user, Cham (2017)
\bibitem{Cristiani2011} E. Cristiani, B. Piccoli, A. Tosin: Multiscale modeling of granular flows with application to crowd dynamics. Multiscale Modeling and Simulation, \textbf{9}(1), pp. 155-182 (2011)
\bibitem{Piccoli2009} B. Piccoli, A. Tosin: Pedestrian flows in bounded domains with obstacles. Continuum Mechanics and Thermodynamics, \textbf{21}, pp. 85-107 (2009)
\bibitem{Zuriguel2014} I. Zuriguel, D. R. Parisi, R. C. Hidalgo, C. Lozano, A. Janda, P. A. Gago, J. P. Peralta, L. M. Ferrer, L. A. Pugnaloni, E. Cl\'{e}ment, D. Maza, I. Pagonabarraga, A. Garcimart\'{i}n: Clogging transition of many-particle systems flowing through bottlenecks. Scientific Reports, \textbf{4}, 7324 (2014)
\bibitem{Garcimartin2015} A. Garcimart\'{i}n, J. M. Pastor, L. M. Ferrer, J. J. Ramos, C. Mart\'{i}n-G\'{o}mez, I. Zuriguel: Flow and clogging of a sheep herd passing through a bottleneck. Physical Review E, \textbf{91}, 022808 (2015)
\bibitem{OmarMSC} O.  Richardson: Large-scale multiscale particle models in inhomogeneous domains: modelling and implementation. Master thesis (2016) \url{https://arxiv.org/abs/1609.03732} 
\bibitem{Faure2015} S. Faure, B. Maury: Crowd motion from the granular stand point. Mathematical Models and Methods in Applied Sciences, \textbf{25} pp. 463-493 (2015)
\bibitem{Bortz} A.B.Bortz, M.H.Kalos, J.L.Lebowitz: New algorithm for Monte Carlo simulations of Ising spin systems. J. Comp. Phys. \textbf{17}, pp. 10-18 (1975)
\bibitem{Kratzer} P. Kratzer: Monte Carlo and Kinetic Monte Carlo. Methods -- A Tutorial, in Multiscale Simulation Methods in Molecular Sciences, edited by J. Grotendorst, N. Attig, S. Blügel, and D. Marx, NIC Series (Forschungszentrum Jülich), \textbf{42}, pp. 51-76 (2009)


% Journal article
%\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%%
%% Journal article by DOI
%\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%%
%\bigskip
%
%% Use the following (APS) syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Mathematics, Physics, Statistics, Computer Science"
%%
%% Online Document
%\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%%
%% Monograph
%\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%%
%% Journal article
%\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%%
%% Journal article by DOI
%\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%%
%% Contribution 
%\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%%
%\bigskip
%%
%% Use the following syntax and markup for your references if 
%% the subject of your book is from the field 
%% "Psychology, Social Sciences"
%%
%%
%% Monograph
%\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%%
%% Online Document
%\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%%
%% Journal article
%\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
%\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
%\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
%\bigskip
%
% Journal article
%\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
%\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
%\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
%\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
%\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O�Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...�': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
%\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
%\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
%\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
%\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
%\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
%\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

